Towards Adversarial Configurations for Software Product Lines

Ensuring that all supposedly valid configurations of a software product line (SPL) lead to well-formed and acceptable products is challenging since it is most of the time impractical to enumerate and test all individual products of an SPL. Machine learning classifiers have been recently used to predict the acceptability of products associated with unseen configurations. For some configurations, a tiny change in their feature values can make them pass from acceptable to non-acceptable regarding users' requirements and vice-versa. In this paper, we introduce the idea of leveraging these specific configurations and their positions in the feature space to improve the classifier and therefore the engineering of an SPL. Starting from a variability model, we propose to use Adversarial Machine Learning techniques to create new, adversarial configurations out of already known configurations by modifying their feature values. Using an industrial video generator we show how adversarial configurations can improve not only the classifier, but also the variability model, the variability implementation, and the testing oracle.

==> motivating_example.tex <==
\section{Motivating examples and Problem statement}
\label{sec:motiv}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MOVE SECTION 2 (FRAMEWORK) (more or less)
%%What do JHipster, the Linux Kernel and a video generator have in common?
%%A priori not much, they are related to rather different domains (respectively web application, OS and videos/Computer Vision/Image Processing), they are written in different languages(respectively Java, C/C++ and Lua or others), they defined different number of options(respectively about 50, 13,000 and 80) of different types (mostly boolean, mostly boolean and tri-state or real values).
%%Yet, they all are considered as Software Product Lines.
%What do Software Product Lines have in common?
%Usually, SPLs are composed of a Variablity Model defining variability points, features represented on a hierarchical fashion; but also value ranges and constraints defining, first, the valid values that features can take and, second, the association of features that are considered valid or not.
%Features are also mapped to pieces of code.
%Finally, usually a SPL is associated to an oracle which defines, represents and formulates users' needs.
%Usually, an oracle is a redundant and time-consuming task that can be decomposed into: selecting features and their values; compose the different parts of code associated to selected features; build the resulting program; execute it on specific inputs to check whether it complies with specific needs.
%Thus, it is advantageous to automate this process.
%%It is an automatic procedure that states whether a configuration complies with expressed needs.
%%Usually, this task is decomposed into: selecting features and their values; compose the different parts of code associated to selected features; build the resulting program; execute it on specific inputs to check whether it complies with specific needs.

%Even if the process is automated, it remains time and energy consuming.
%Therefore, an other way is needed to reduce computations and save time to predict the result of the oracle.
%It is usually assumed that a small change in a configuration does not lead to chaotic response from the oracle.
%That is: knowing the response of the oracle regarding a specific program variant and thus its configuration, a neighbor configuration, differing only in a few amount for a few features, should be the same.
%This assumption allows to use Machine Learning technique to generalize a decision made on a known configuration to never-seen-before configuration but that lies in a "close" neighborhood.

%Using Machine Learning techniques implies training a classifier that will act like the oracle but much faster.
%The classifier will only consider the configuration and the knowledge learnt from examples given in the training set to decide whether the configuration is likely to meet users' needs or not.
%Using these techniques, the classifier is supposed to be strong enough to give similar results as if the evaluation would have used the oracle, however, there is no need to derive the configuration into an actual program variant and to measure its performance.

%However, because the classifier is based on statistical approaches and it does not hold all the required knowledge, it can make prediction mistakes, after being trained.
%Consequences can be dramatic as, considering a Computer Vision system that is embedded in autonomous cars, if the configuration cannot comply with all requirements it could lead to tragic lethal accidents.
%On a less tragic note, in the industry, it is well-known that fixing a mistake costs much as it is discovered latter in the process.
%By the time the decision mistake is discovered, the configuration is already deployed.
%Fixing this error implies to reconfigure the system which might involve shutting it down for a moment and then restarting it again.
%In the end, it results in a loss of money and energy for the company.

% \begin{figure}
% \centering
% \includegraphics[scale=0.25]{Images/diff_gt_class.png}
% \label{fig:classif_errors}
% \caption{An 2D example of our different the classifier function (red line) and the ground truth (blue line) might be. The classifier needs training examples represented by points and their colors stating for their classes. The classification of P3 is strong as it is deep into the orange (upper right corner) class while the confidence in P2 and P1 becomes lower as they get closer to the classifier function.}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END MOVE SECTION 2 (FRAMEWORK)

Now that we have presented entities traditionally forming SPLs and why ML techniques could be useful, we will instance the use of ML techniques to different SPLs, detail the characteristics of the latter, detail the advantages of using ML techniques in such context and the benefits of trying to reduce differences between classifier functions and oracles.

% \textbf{JHipster}
% JHipster is an open-source, industrially used generator for developing Web applications.
% The project is now popular with more than $6,000$ stars on Github and gather around 300 contributors.
% JHipster generates a full-stack web application (using various technologies such as Angular, Bootstrap, MongoDB, authentification techniques, etc.) out of a user-specified configuration.
% A configuration can define nearly $50$ configuration options in order to build an application that fits users' needs.
% Not all combination of possible and JHipster already provides some constraints.
% On the other hand, because it manages various technologies, it also deals with different programming languages (such as Java, CSS, SQL, etc.).
% All of that makes JHipster an interesting tool with enough complexity to motivate the use of ML techniques.

% Furthermore, from a user perspective, goals and concerns may vary from one user to another.
% For instance, one user might want to build an application that will scale in terms of databases requests while an other might want to minimize the memory taken by the generated stack.\\


\textbf{Video generator}
\label{sec:video_gen}
\cite{temple:hal-01323446} has used an industrial video generator. Again, it is composed of two parts:
a VM that abstractly describes configuration options impacting the characteristics of generated videos (\eg is there fog or blur? Is there noise? Dynamic or static noise? How many moving objects? What are their paths? etc.). In total, 80 configuration options are taken into account. Among them, a few are boolean, the rest are categorical (an enumeration) or real-value options. \cite{temple:hal-01323446} described some of the constraints that were already implemented in the VM and thanks to ML add others such as the interaction between noise and blur.

The second part is the generator that will take as input a configuration file and produce a video file.
It is implemented in Lua.

Again, from a user perspective, various goals and concerns can be defined.
For instance, generated videos can be used to test Computer Vision based systems, thus, these videos must be challenging in some way: there is a lot of noise or blur in some of them; some additional moving objects can be used in order to make the tracking of objects difficult, etc.
There might be also some requirements in terms of the size of the output video as dynamic noise is difficult to encode, introducing some will increase the size of the video in the end while using blur is likely to reduce it (as portions of images will be uniform).\\


For all those reasons, it is important to be sure that the classifier does not have "blind spots" and that the decisions it makes are as close as possible from the decision that the oracle could make.
Said differently, we want to reduce the number of errors made by the classifier with regards to the oracle or we want to fit the decision function of the classifier to the one given by the oracle.


